Security and Privacy of IP-ICN Coexistence: A Comprehensive Survey

Today Internet is experiencing a massive number of users with a continuously increasing need for data, which is the leading cause of introduced limitations among security and privacy issues. To overcome these limitations, a shift from host-centric to data-centric is proposed, and in this context, Information-Centric Networking (ICN) represents a promising solution. Nevertheless, unsettling the current Internet network layer, i.e., Internet Protocol (IP), with ICN is a challenging, expensive task since it requires worldwide coordination among Internet Service Providers (ISPs), backbone, and Autonomous Services (AS). Therefore, researchers foresee that the replacement process of the current Internet will transition through the coexistence of IP and ICN. In this perspective, novel architectures combine IP and ICN protocols. However, only a few of the proposed architectures place the security-by-design feature. Therefore, this article provides the first comprehensive Security and Privacy (SP) analysis of the state-of-the-art IP-ICN coexistence architectures by horizontally comparing the SP features among three deployment approaches, i.e., overlay, underlay, and hybrid, and vertically comparing among the ten considered SP features. Lastly, the article sheds light on the open issues and possible future directions for IP-ICN coexistence. Our analysis shows that most architectures fail to provide several SP features, including data and traffic flow confidentiality, availability, and anonymity of communication. Thus, this article shows the secure combination of current and future protocol stacks during the coexistence phase that the Internet will definitely walk across.

==> tables/all-architectures-evaluation.tex <==
%\begin{landscape}
\begin{table*}[!htb] 
%\tiny
\centering
%\caption{Evaluation of S\&P features for coexistence architectures}
\caption{Evaluation of Security and Privacy features of current IP/ICN coexistence architectures.}
\label{tab: evaluation}
\scalebox{0.9}{
\begin{tabular}{p{4cm} c c c c c c c c c c c c c c c c c c c c}
  \toprule
  %\hline
  \centering \textbf{SP Feature} & 
  \textbf{\rotatebox{90}{\scriptsize PURSUIT~\cite{pursuit}}} & 
  \textbf{\rotatebox{90}{\scriptsize NetInf~\cite{netinf}}} & 
  \textbf{\rotatebox{90}{\scriptsize NDN~\cite{ndn}}} &
  \textbf{\rotatebox{90}{\scriptsize NDNFlow~\cite{ndnflow}}} &
  \textbf{\rotatebox{90}{\scriptsize O-ICN~\cite{oicn}}} &
  \textbf{\rotatebox{90}{\scriptsize CONET~\cite{conet}}} &
  \textbf{\rotatebox{90}{\scriptsize GreenICN~\cite{greenICN}}} &
  \textbf{\rotatebox{90}{\scriptsize coCONET~\cite{coCONET}}} &
  \textbf{\rotatebox{90}{\scriptsize OpenFlow-ICN~\cite{openflowicn}}} &
  \textbf{\rotatebox{90}{\scriptsize SDN-PURSUIT~\cite{SDNPURSUIT}}} &
  \textbf{\rotatebox{90}{\scriptsize IICN~\cite{iicn}}} &
  \textbf{\rotatebox{90}{\scriptsize DOCTOR~\cite{doctor}}} & 
  \textbf{\rotatebox{90}{\scriptsize POINT~\cite{point}}} & 
  \textbf{\rotatebox{90}{\scriptsize RIFE~\cite{rife}}} & 
  \textbf{\rotatebox{90}{\scriptsize CableLabs~\cite{cacheLabs}}} &
  \textbf{\rotatebox{90}{\scriptsize COIN~\cite{coin}}} &
  \textbf{\rotatebox{90}{\scriptsize NDN-LAN~\cite{ndnLAN}}} & 
  \textbf{\rotatebox{90}{\scriptsize hICN~\cite{hICN}}} & 
  \textbf{\rotatebox{90}{\scriptsize OFELIA~\cite{ofelia}}} & 
  \textbf{\rotatebox{90}{\scriptsize CLIP~\cite{clip}}} \\
  \toprule 
   %\hline
   %\multirow{10}*{SP Features} & 
   \makecell{ Trust} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{360} \\
    \hline
    \makecell{Data origin authentication} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{360} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} \\
    \hline
    \makecell{Peer entity authentication}& \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180}  & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} \\
    \hline
    \makecell{Data integrity} & \tiny \pie{180} & \tiny \pie{360} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{360} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} \\   
    \hline
    \makecell{Authorization \& access control} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} &  \tiny \pie{0} & \tiny \pie{180} \\
    \hline
    \makecell{Accountability} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{360} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0}\\
    \hline
    \makecell{Data confidentiality} & \tiny \pie{0} & \tiny \pie{0} &  \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{0}  & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{360} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0}\\
    \hline
    \makecell{Availability} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0}\\
    \hline
    \makecell{Anonymous  communication} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} \\
    \hline
    \makecell{Traffic flow  confidentiality} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0}  & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0}\\
    %\hline
    %\makecell{Anonymous  communication} & \tiny \pie{360} & \tiny \pie{360} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{0} & \tiny \pie{180} & \tiny \pie{180} & \tiny \pie{0} \\
 
\bottomrule
\end{tabular}}
\\[1\baselineskip]
\tiny \pie{360} \scriptsize Fulfilled~~~~~~ \tiny \pie{180} \scriptsize{Partially fulfilled}~~~~~~\tiny \pie{0} Not fulfilled
\end{table*}

==> tables/discussion-additional-technologies.tex <==
\begin{table*}[!ht] 
%\tiny
\centering
%\caption{Evaluation of S\&P features for coexistence architectures}
\caption{Summary of the additional technologies used for each deployment approach.}
\label{tab:additional-technologies}
    \begin{tabular}{ c c c  c  c c c c c c c}
      \toprule
      %\hline
       \makecell{\multirow{3}{*}{Deployment approach}} &
       \multirow{3}{*}{\makecell{Analysed \\ architectures}} &
       \multicolumn{5}{c}{Deployment scenario} &
       \multicolumn{4}{c}{Additional technologies} \\
       \cline{3-11}\\
       & & \makecell{ICN-ICN \\ in IP} & \makecell{ICN-IP \\ in IP} & \makecell{ICN-IP \\ in ICN} & \makecell{IP-IP \\ in ICN} & \makecell{Border \\ Island} & \makecell{SDN} & \makecell{CDN} & \makecell{DTN} & \makecell{NFV} \\
      \toprule 
       \makecell{Overlay} & 10 & 10 & 4 & 0 & 0 & 0 & 6 & 0 & 0 & 0 \\
        \midrule
        \makecell{Underlay} & 6 & 4 & 4 & 3 & 3 & 4 & 2 & 2 & 1 & 1\\
        \midrule
        \makecell{Hybrid} & 4 & 3 & 3 & 3 & 3 & 2 & 0 & 0 & 0 & 0 \\
        
    \bottomrule
    \end{tabular}
\end{table*}

==> tables/icn-ip-sdn.tex <==
\begin{table*}[t]
    \caption{SP feature overview for IP/IPSec and ICN/NDN protocols.}
    \centering
        \begin{tabular}{ c | c  c  c}
            \toprule
            Feature & Protocol & Support & Mechanism \\ %& Related SP issues \\
            \midrule
            \multirow{2}{*}{Trust} & IP/IPSec & \checkmark  & Public Key Infrastructure \\ % &  IP/MAC Spoofing \\
             &  ICN/NDN & \checkmark & Certificates \\ % & Content poisoning \\
             %& SDN & \checkmark & & Data Confidentiality\\
             %& CDN & \checkmark & & Data Confidentiality\\
            \midrule
            \multirow{2}{*}{Data origin authentication and integrity} & IP/IPSec & \checkmark & HMAC~\cite{krawczyk1997hmac} \\ %& None \\
             & ICN/NDN & $\circ$ & Producer's signature \\ %& (Partial) Modification, Repudiation \\
            \midrule
            %\multirow{2}{*}{Data integrity} &  IP/IPSec  & Host-based communication & & Data Origin Authentication \\
            % & ICN/NDN & Control plane & & Data Integrity  \\
            %\midrule 
            \multirow{2}{*}{Peer entity authentication} &  IP/IPSec  & \checkmark & Shared keys and signature \\ %& None\\
             & ICN/NDN & \xmark & None \\ %& Unauthorized entities\\
             \midrule
            \multirow{2}{*}{Authorization \& access control} &  IP/IPSec  & $\circ$ & Access Control Lists \\ %& IP spoofing, Unauthorized access \\
             & ICN/NDN & \xmark & None \\ %& Unauthorized access \\
              \midrule
            \multirow{2}{*}{Accountability} &  IP/IPSec  & \checkmark & Egress filter \\ %& IP spoofing \\
             & ICN/NDN & $\circ$ & Producer's signature \\ %& (Partial) Non traceability \\
              \midrule
            \multirow{2}{*}{Data confidentiality} &  IP/IPSec  & \checkmark & ESP header \\ %& Traffic Analysis\\
             & ICN/NDN & $\circ$ & Encryption \\ %& Traffic Analysis, Name Privacy\\
              \midrule
            \multirow{2}{*}{Availability} &  IP/IPSec  & \xmark & None \\ %& DoS and DDoS\\
             & ICN/NDN & \xmark & None \\ %& DoS and DDoS\\
              \midrule
            \multirow{2}{*}{Anonymous communication} &  IP/IPSec  & $\circ$ & Tunnel mode \\ %& Privacy attacks\\
             & ICN/NDN & $\circ$ & Consumer's anonymity by design \\  %& Privacy attacks \\
              \midrule
            \multirow{2}{*}{Traffic flow confidentiality} &  IP/IPSec  & $\circ$ & Padding \\ %& Side-channel \\
             & ICN/NDN & \xmark & None \\ %& Side-channel\\
            \bottomrule
        \end{tabular}
    \label{tab:feature-overview}
\end{table*}

==> tables/new-background-table.tex <==
\begin{table*}[!ht]
    \caption{Overview of the protocols that are used to enable IP-ICN coexistence. \textcolor{blue}{The table summarizes the type of the current deployment of the described protocols -- i.e., deployment type --, their general characteristics regarding the communication model and other protocol-oriented attributes --i.e., general features --, and the security and privacy features guaranteed by design---i.e., SP features.}}
    \centering
        \begin{tabular}{ c c  c c c c c}
            \toprule
            \multirow{2}{*}{\textbf{Protocol}} & \multirow{2}{*}{\textbf{Deployment Type}} & \multirow{2}{*}{\textbf{General Features}} & \multicolumn{4}{c}{\textbf{SP Features}} \\
            \cmidrule{4-7}
            & & & \makecell{Data Origin \\ Authentication} & \makecell{Data \\ Integrity} & \makecell{Data \\ Confidentiality} & \makecell{Consumer \\ Anonymity} \\
            \midrule
            \multirow{3}{*}{IP/IPSec} & \multirow{3}{*}{Clean slate} & \makecell{Host-based communication \\ IPv4 \& IPv6 \\ IPSec: AH and ESP} & \multirow{5}{*}{\thead[c]{Message Authentication Code \\ (MAC) verification via \\ shared secret keys \\ for each packet}} & & &\\
            \cmidrule{1-3}
            \makecell{SDN} & \makecell{Overlay in IP} & \makecell{Host-based communication \\ Centralized network\\ Control and data plane decoupling \\ Improved network management} & & & & \\
            \cmidrule{1-3}
            \makecell{CDN} & \makecell{Overlay in IP} & \makecell{Host-based communication \\ Efficient content distribution \\ Improved content availability} & & & &  \\
            \cmidrule{1-3}
            \makecell{NFV} & \makecell{Overlay in IP} & \makecell{Host-based communication \\ Hardware and software decoupling \\ Flexible and scalable networks} & & & &\\
            \cmidrule{1-3}
            \makecell{DTN} & \makecell{Overlay in IP} & \makecell{Host-based communication \\ Delay- tolerant applications} & & & &\\
            \midrule
            \makecell{ICN} & \makecell{Clean slate} & \makecell{Content-based communication \\ Content-based security \\ In-network caching \\ Name-based forwarding} & & & & \\
            \bottomrule
        \end{tabular}
    \label{tab:background}
\end{table*}
